Herding LLaMaS: Using LLMs as an OS Module

Computer systems are becoming increasingly heterogeneous with the emergence of new memory technologies and compute devices. GPUs alongside CPUs have become commonplace and CXL is poised to be a mainstay of cloud systems. The operating system is responsible for managing these hardware resources, requiring modification every time a new device is released. Years of research and development are sunk into tuning the OS for high performance with each new heterogeneous device. With the recent explosion in memory technologies and domain-specific accelerators, it would be beneficial to have an OS that could provide high performance for new devices without significant effort. We propose LLaMaS which can adapt to new devices easily. LLaMaS uses Large Language Models (LLMs) to extract the useful features of new devices from their textual description and uses these features to make operating system decisions at runtime. Adding support to LLaMaS for a new device is as simple as describing the system and new device properties in plaintext. LLaMaS reduces the burden on system administrators to enable easy integration of new devices into production systems. Preliminary evaluation using ChatGPT shows that LLMs are capable of extracting device features from text and make correct OS decisions based on those features.

==> text/2_Background.tex <==
\section{Large Language Models (LLMs)}
\begin{enumerate}
    \item Brief background of LLMs. Papers where LLMs are used as decision making engines.
\end{enumerate}



==> text/N_LookingAhead.tex <==
\section{Looking ahead}
What we foresee in the future.
